Passively Measuring IPFS Churn and Network Size

The InterPlanetary File System~(IPFS) is a popular decentralized peer-to-peer network for exchanging data. While there are many use cases for IPFS, the success of these use cases depends on the network. In this paper, we provide a passive measurement study of the IPFS network, investigating peer dynamics and curiosities of the network. With the help of our measurement, we estimate the network size and confirm the results of previous active measurement studies.

==> con_versions <==
agent, share
missing, 3059
0.10.0, 8800
0.11.0, 2898
0.11.0-dev, 117
0.4.21, 639
0.4.22, 178
0.4.23, 1016
0.5.0-dev, 125
0.6.0, 200
0.7.0, 11222
0.8.0, 19536
0.9.0, 2754
0.9.1, 2314
ant/0.2.1/fe027af, 273
go-qkfile/0.9.1/, 1319
hydra-booster/0.7.4, 1028
ioi, 6958
ipfs\_crawler, 228
nebula-crawler, 321
other, 767
storm, 2101

